Time-Warping Recurrent Neural Networks for Transfer Learning

Dynamical systems describe how a physical system evolves over time. Physical processes can evolve faster or slower in different environmental conditions. We use time-warping as rescaling the time in a model of a physical system. This thesis proposes a new method of transfer learning for Recurrent Neural Networks (RNNs) based on time-warping. We prove that for a class of linear, first-order differential equations known as time lag models, an LSTM can approximate these systems with any desired accuracy, and the model can be time-warped while maintaining the approximation accuracy. The Time-Warping method of transfer learning is then evaluated in an applied problem on predicting fuel moisture content (FMC), an important concept in wildfire modeling. An RNN with LSTM recurrent layers is pretrained on fuels with a characteristic time scale of 10 hours, where there are large quantities of data available for training. The RNN is then modified with transfer learning to generate predictions for fuels with characteristic time scales of 1 hour, 100 hours, and 1000 hours. The Time-Warping method is evaluated against several known methods of transfer learning. The Time-Warping method produces predictions with an accuracy level comparable to the established methods, despite modifying only a small fraction of the parameters that the other methods modify.

==> metainfo.tex <==
\makeatletter
% \title{\textbf{\uppercase{Time-Warping Recurrent Neural Networks for Transfer Learning}}}
\title{Time-Warping Recurrent Neural Networks for Transfer Learning}
 
\authorLast{Hirschi}
\authorFirst{Jonathon}
\authorMiddle{Michael}
\education{
B.S., University of British Columbia, 2016 \\
M.S., University Colorado Denver, 2024
}


\school{University of Colorado Denver}
\program{Applied Mathematics}
\reportType{dissertation} %edited. Other options: dissertation, thesis
\degreeName{Doctor of Philosophy} %edited. Other options: Doctor of Philosophy

%Set the following 3 variables for your Date of graduation
\submitDay{22}
\submitMonth{April}
\submitYear{2026}

%Set the following variables to define your advisor and committee members
\advisor{Jan Mandel}
\advisorTitle{Dr.}
\committeeChair{Joshua French}
\committeeMembers{
Kyle Hilburn, \\ 
Angel Farguell, \\
Farhad Pourkamali
}

%Setting the PDF metadata via the hyperref package.
%Please do not edit below unless you really know what you are doing.
\hypersetup{
    pdftitle={\@title},
    pdfsubject={\@degreeName\ \@reportType (\@submitDay\ \@submitMonth\ \@submitYear)},
    pdfauthor={\@authorFirst\ \@authorLast }
}
